Achieving Constant Regret in Linear Markov Decision Processes

We study the constant regret guarantees in reinforcement learning (RL). Our objective is to design an algorithm that incurs only finite regret over infinite episodes with high probability. We introduce an algorithm, Cert-LSVI-UCB, for misspecified linear Markov decision processes (MDPs) where both the transition kernel and the reward function can be approximated by some linear function up to misspecification level $\zeta$. At the core of Cert-LSVI-UCB is an innovative \method, which facilitates a fine-grained concentration analysis for multi-phase value-targeted regression, enabling us to establish an instance-dependent regret bound that is constant w.r.t. the number of episodes. Specifically, we demonstrate that for a linear MDP characterized by a minimal suboptimality gap $\Delta$, Cert-LSVI-UCB has a cumulative regret of $\tilde{\mathcal{O}}(d^3H^5/\Delta)$ with high probability, provided that the misspecification level $\zeta$ is below $\tilde{\mathcal{O}}(\Delta / (\sqrt{d}H^2))$. Here $d$ is the dimension of the feature space and $H$ is the horizon. Remarkably, this regret bound is independent of the number of episodes $K$. To the best of our knowledge, Cert-LSVI-UCB is the first algorithm to achieve a constant, instance-dependent, high-probability regret bound in RL with linear function approximation without relying on prior distribution assumptions.

==> tables.tex <==
\begin{table}[!htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline 
C. & Q. & $\zeta = 0.0$ & 0.01 & 0.02 & 0.03 & 0.04\\
\hline
$\times$ & $\times$ & 189.01 $\pm$ \small{57.21} & 190.57 $\pm$ \small{59.49} & \textbf{194.74} $\pm$ \small{61.99} & \textbf{201.36} $\pm$ \small{63.67} & \textbf{211.67} $\pm$ \small{66.06} \\
$\times$ & $\checkmark$ & \textbf{189.00} $\pm$ \small{57.18} & \textbf{190.55} $\pm$ \small{59.49} & 194.75 $\pm$ \small{61.99} & 201.41 $\pm$ \small{63.67} & 211.68 $\pm$ \small{66.06}\\
$\checkmark$ & $\times$ & 196.32 $\pm$ \small{64.09} & 203.68 $\pm$ \small{77.24} & 200.41 $\pm$ \small{66.88} & 207.47 $\pm$ \small{70.97} & 222.61 $\pm$ \small{78.77}\\
$\checkmark$ & $\checkmark$ & 196.31 $\pm$ \small{64.06} & 199.07 $\pm$ \small{68.45} & 200.42 $\pm$ \small{66.88} & 207.52 $\pm$ \small{70.96} & 222.62 $\pm$ \small{78.77}\\
\hline
\end{tabular}
}
\vskip 0.5em
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
C. & Q. & $\zeta = 0.05$ & 0.06 & 0.07 & 0.08 & 0.09\\
\hline
$\times$ & $\times$ & 220.52 $\pm$ \small{67.85} & 233.57 $\pm$ \small{66.54} & 248.08 $\pm$ \small{68.70} & 264.49 $\pm$ \small{72.05} & 279.82 $\pm$ \small{78.28}\\
$\times$ & $\checkmark$ & \textbf{220.50} $\pm$ \small{67.86} & 233.48 $\pm$ \small{66.50} & \textbf{248.06} $\pm$ \small{68.69} & 264.56 $\pm$ \small{72.00} & 279.81 $\pm$ \small{78.25}\\
$\checkmark$ & $\times$ & 221.87 $\pm$ \small{73.51} & 232.75 $\pm$ \small{73.75} & 261.16 $\pm$ \small{84.44} & \textbf{262.07} $\pm$ \small{82.05} & 273.56 $\pm$ \small{96.19}\\
$\checkmark$ & $\checkmark$ & 221.86 $\pm$ \small{73.51} & \textbf{232.70} $\pm$ \small{73.81} & 261.14 $\pm$ \small{84.43} & 262.15 $\pm$ \small{82.01} & \textbf{273.55} $\pm$ \small{96.17}\\
\hline
\end{tabular}
}
\vskip 0.5em
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
C. & Q. & $\zeta=$0.1 & 0.11 & 0.12 & 0.13 & 0.14 \\
\hline
$\times$ & $\times$ & 292.59 $\pm$ \small{80.52} & 305.73 $\pm$ \small{83.47} & 323.93 $\pm$ \small{90.25} & 337.65 $\pm$ \small{94.39} & 355.49 $\pm$ \small{106.22}\\
$\times$ & $\checkmark$ & 292.68 $\pm$ \small{80.55} & 305.71 $\pm$ \small{83.44} & 323.91 $\pm$ \small{90.23} & 337.65 $\pm$ \small{94.39} & 355.49 $\pm$ \small{106.22}\\
$\checkmark$ & $\times$ & \textbf{285.81} $\pm$ \small{102.54} & 297.98 $\pm$ \small{107.21} & 315.22 $\pm$ \small{114.50} & \textbf{335.69} $\pm$ \small{110.76} & \textbf{339.81} $\pm$ \small{99.26}\\
$\checkmark$ & $\checkmark$ & 285.90 $\pm$ \small{102.57} & \textbf{297.97} $\pm$ \small{107.18} & \textbf{315.20} $\pm$ \small{114.49} & 335.69 $\pm$ \small{110.76} & 339.82 $\pm$ \small{99.27}\\
\hline
\end{tabular}
}
\vskip 0.5em
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
C. & Q. & $\zeta=$0.15 & 0.2 & 0.25 & 0.3 & Time(s) \\
\hline
$\times$ & $\times$ & 377.27 $\pm$ \small{127.21} & 450.49 $\pm$ \small{154.80} & 526.45 $\pm$ \small{181.90} & 634.46 $\pm$ \small{245.70} & 1654.76 $\pm$ \small{125.40} \\
$\times$ & $\checkmark$ & 377.23 $\pm$ \small{127.13} & 450.48 $\pm$ \small{154.79} & \textbf{526.36} $\pm$ \small{181.91} & 634.48 $\pm$ \small{245.68} & 1654.21 $\pm$ \small{141.31} \\
$\checkmark$ & $\times$ & 351.52 $\pm$ \small{118.09} & 436.30 $\pm$ \small{154.89} & 530.15 $\pm$ \small{194.89} & \textbf{605.64} $\pm$ \small{233.19} & 1599.66 $\pm$ \small{138.18} \\
$\checkmark$ & $\checkmark$ & \textbf{351.50} $\pm$ \small{118.03} & \textbf{436.29} $\pm$ \small{154.91} & 530.58 $\pm$ \small{195.24} & 605.67 $\pm$ \small{233.18} & \textbf{1593.38} $\pm$ \small{98.11}\\
\hline
\end{tabular}
}
\vskip 0.5em
\caption{Average cumulative regret {\small{($\pm$ standard derivation)}} and execution time over 2000 episodes. The results are averaged over 16 individual runs. \textbf{C} indicates if Certified Estimator is used. \textbf{Q} indicates if Quantization is used.} \label{tab:1}
\end{table}
\begin{figure}
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{nips2024/overall-cropped.pdf}
         \caption{With quantization}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{nips2024/overall_f-cropped.pdf}
         \caption{Without quantization}
         \label{fig:three sin x}
     \end{subfigure}
        \caption{Cumulative regret over 2000 episodes with respect to different misspecification level $\zeta$. The result is averaged over 16 individual environments. }
        \label{fig:1}
\end{figure}
\begin{figure}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{nips2024/0-cropped.pdf}
         \caption{$\zeta = 0$}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{nips2024/0.05-cropped.pdf}
         \caption{$\zeta = 0.05$}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{nips2024/0.1-cropped.pdf}
         \caption{$\zeta = 0.10$}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{nips2024/0.15-cropped.pdf}
         \caption{$\zeta = 0.15$}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{nips2024/0.2-cropped.pdf}
         \caption{$\zeta = 0.20$}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{nips2024/0.25-cropped.pdf}
         \caption{$\zeta = 0.25$}
     \end{subfigure}
        \caption{Cumulative regret with respect to the number of episodes. We reported the median cumulative regret with the shadow area as the region from 25\% percentage to 75\% percentage statistics over 16 runs. }
        \label{fig:2}
\end{figure}
% \end{document}

